2D and 3D Vascular Structures Enhancement via Multiscale Fractional Anisotropy Tensor

The detection of vascular structures from noisy images is a fundamental process for extracting meaningful information in many applications. Most well-known vascular enhancing techniques often rely on Hessian-based filters. This paper investigates the feasibility and deficiencies of detecting curve-like structures using a Hessian matrix. The main contribution is a novel enhancement function, which overcomes the deficiencies of established methods. Our approach has been evaluated quantitatively and qualitatively using synthetic examples and a wide range of real 2D and 3D biomedical images. Compared with other existing approaches, the experimental results prove that our proposed approach achieves high-quality curvilinear structure enhancement.

==> tex/ROC-3d.tex <==
\begin{figure}[h!]
	\centering
	\begin{subfigure}{.35\linewidth}
		\begin{tikzpicture}
		\begin{axis}[
		width = 1.2\linewidth,
		xlabel={False Positive Rate (1-Specificity)},
		ylabel={True Positive Rate (1-Sensitivity)},
		ylabel near ticks,
		label style={font=\footnotesize},
		tick label style={font=\footnotesize},
		ytickmin=0, ymax=1.05,
		xtickmin=0, xtickmax=1.05,
		enlargelimits=false,
		legend entries = {Raw image, Vesselness, Neuriteness, PCT ves., PCT neu., RVR, $V_{FAT}$,$V_{PFAT}$},
		legend columns = 1,
		legend style={font=\footnotesize,line width=2pt, draw=none,},
		legend to name=leg3D,
		grid=major, % Display a grid
		grid style={dashed,gray!30}, % Set the style
		]
		\addplot[color=black,loosely dashed] table [x index=0, y index=1, col sep=comma] {images/datFiles/vascuO.dat};%Raw Image
		\addplot[color=brewerDark1,line width=1pt] table [x index=0, y index=1, col sep=comma] {images/datFiles/vascuV.dat};%Vesselness
		\addplot[color=brewerDark2,line width=1pt] table [x index=0, y index=1, col sep=comma] {images/datFiles/vascuN.dat};%Neuriteness
        \addplot[color=brewerDark3,line width=1pt] table [x index=0, y index=1, col sep=comma] {images/datFiles/vascuPctV.dat};%PCT Vesselness
		\addplot[color=brewerDark4,line width=1pt] table [x index=0, y index=1, col sep=comma] {images/datFiles/vascuPctN.dat}; % PCT Neuriteness	
	   \addplot[color=brewerDark5,line width=1pt] table [x index=0, y index=1, col sep=comma] {images/datFiles/vascuVR.dat}; % VR	
	   \addplot[color = red,line width=1pt] table [x index=0, y index=1, col sep=comma] {images/datFiles/vascuE.dat};% proposedE
	    \addplot[color = black,line width=1pt] table [x index=0, y index=1, col sep=comma] {images/datFiles/vascuP.dat};% proposedP
		\end{axis}
		\end{tikzpicture}
	\end{subfigure}\quad \quad
	\begin{subfigure}{.25\linewidth}
		\vskip-4pt
	\centering
	\pgfplotslegendfromname{leg3D}
\end{subfigure}

\caption{Mean ROC curve for all the 9 vascular networks 3D images enhanced using the state-of-the-art approaches alongside the proposed method (see legend for colours). Correspondingly, the mean AUC values can be found in Table~\ref{tab:auc3}.}\label{fig:roc:vascu}
\end{figure}

==> tex/acknowlegde.tex <==

\section{Acknowlegdement}
Haifa F. Alhasson and Shuaa S. Alharbi are supported by the Saudi Arabian Ministry of Education Doctoral Scholarship and Qassim University in Saudi Arabia.

==> tex/future.tex <==
\section{Future work}
Future extension of this work will be development of an enhancement method that improves the result of ridge detection process, exploration of local kernel-based adaptation approaches such as: (curved-support and anisotropic Gaussian) with Hessian-based approaches which provide unified response across all curve-like features to overcome the deficiencies of both classes such as: lack intensity on the junctions, background noise, sensitivity to intensities inhomogeneities and contrast which are main challenges in curve-like enhancement field.



==> tex/keyword.tex <==
\keywords{Curvilinear Structures  \and Curvilinear Enhancement \and Fractional Anisotropy tensor.}

==> tex/table-Vascular-3d.tex <==
%------------Table------------------%

\begin{table}[hb!]
\caption{AUC values for the 9 vascular networks 3D images with increasing network complexity (see Fig.~\ref{fig:vascu:input}) enhanced with the state-of-the-art approaches alongside the proposed method.}\label{tab:auc3}
	\centering
	
	\begin{adjustbox}{width=.97\linewidth}
       %\resizebox{.65\textwidth}{!}{
		\begin{tabular}{cccccccc}\toprule
			&\multicolumn{6}{c}{AUC}\\ \cmidrule(l){2-7}\cmidrule(l){2-8}
			{Nodes}	&Vesselness~\cite{frangi1998multiscale}&Neuriteness~\cite{meijering2004design}&PCT ves.~\cite{sazak2017contrast}& PCT neu.~\cite{sazak2017contrast} &RVR~\cite{jerman2016enhancement} & ${\overline{MFAT}_{\lambda}}$ (Ours) &${\overline{MFAT}_{p}}$ (Ours)\\
			\midrule
			5			&0.999	&0.923&	0.840 &0.897&0.999&0.971&0.971\\
			\midrule
			10			&0.996	&0.883&	0.820 &0.873&0.998&0.976&0.977\\
			\midrule
			50			&0.976	&0.830& 0.794 &0.851&0.981&0.986&0.982\\
			\midrule
			100			&0.951	&0.778& 0.778&0.827&0.957&0.984&0.986\\
			\midrule
			200 		&0.930	&0.755& 0.770 &0.799&0.936&0.985&0.985\\
			\midrule
			400			&0.910	&0.746& 0.749 &0.788&0.917&0.985&0.985\\
			\midrule
			600			&0.902	&0.743& 0.742 &0.777&0.909&0.985&0.985\\
			\midrule
			800			&0.885	&0.719&	0.724 &0.756&0.893&0.985&0.985\\
			\midrule
			1000		&0.884	&0.722&	0.726 &0.759&0.891&0.985&0.985\\
			\midrule
			mean (StDev)	&0.937 (0.045)	&0.788 (0.073)& 0.771 (0.040) &0.814 (0.050) &0.942 (0.043) &\textbf{0.982 (0.005)}&\textbf{0.982 (0.005)}\\ 
			\bottomrule
		\end{tabular}
%	}
	\end{adjustbox}
\end{table}

